Reducibility Among Fractional Stability Problems

In this paper, we resolve the computational complexity of a number of outstanding open problems with practical applications. Here is the list of problems we show to be PPAD-complete, along with the domains of practical significance: Fractional Stable Paths Problem (FSPP) [21] - Internet routing; Core of Balanced Games [41] - Economics and Game theory; Scarf's Lemma [41] - Combinatorics; Hypergraph Matching [1]- Social Choice and Preference Systems; Fractional Bounded Budget Connection Games (FBBC) [30] - Social networks; and Strong Fractional Kernel [2]- Graph Theory. In fact, we show that no fully polynomial-time approximation schemes exist (unless PPAD is in FP). This paper is entirely a series of reductions that build in nontrivial ways on the framework established in previous work. In the course of deriving these reductions, we created two new concepts - preference games and personalized equilibria. The entire set of new reductions can be presented as a lattice with the above problems sandwiched between preference games (at the "easy" end) and personalized equilibria (at the "hard" end). Our completeness results extend to natural approximate versions of most of these problems. On a technical note, we wish to highlight our novel "continuous-to-discrete" reduction from exact personalized equilibria to approximate personalized equilibria using a linear program augmented with an exponential number of "min" constraints of a specific form. In addition to enhancing our repertoire of PPAD-complete problems, we expect the concepts and techniques in this paper to find future use in algorithmic game theory.

==> fspp_to_pe.tex <==
Suppose we are given an instance of \fspp, consisting of a set of nodes $V$, a set of preferred paths $\pi(v)$ for all $v \in V$, and a preference relation $\geqprefer_v$ for each set $\pi(v)$. We can also find $\pi(v, S)$, the set of all $P \in \pi(v)$ such that $S$ is a subpath of $P$. Let $q_v(P)$ = the number of paths $Q$ such that $P \geqprefer_v Q$.

We will create the following instance of \pe. The set of players is $V$. The set of strategies $S_v$ for a node $V$ is $\pi(v) \cup \{N\}$ ($N$ stands for ``No path''). For node $v$, there is exactly one edge defined for each strategy. Edge $P'$ for strategy $P = \{S: P \in \pi(v, S)\}$. The edge for strategy $N$ ($N'$) is a singleton edge, containing only that strategy. The payoffs to player $v$ are: $u_v(P') = q_v(P) + 1$, $u_v(N) = 1$.

Suppose $w$ is a set of weights in a personalized equilibrium of the game defined above. $w_v(P')$ represents the weight assigned by $v$ to edge $P'$. We will show that $w$ is a personalized equilibrium if and only if $w': w'_v(P) = w_v(P')$ is a fractionally stable solution to the \fspp\ instance.

First, assume $w$ is a personalized equilibrium. Then, we know that for all $v$, the total weight placed by $v$ on all edges is 1, or $w_v(N) + \sum_{P \in \pi(v)} w_v(P') = 1$. Therefore, $\sum_{P \in \pi(v)} w_v(P') \leq 1 \Rightarrow \sum_{P \in \pi(v)} w'_v(P) \leq 1$, so the Unity condition holds. Also, the sum of weights placed by $v$ on edges adjacent to a strategy $S$ of another player $v'$ is at most $w_{v'}(S)$. That is, for path $S \in \pi(v')$ ($v' \neq v$), $\sum_{P': S \in P'} w_v(P') \leq w_{v'}(S') \Rightarrow \sum_{P \in \pi(v, S)} w_v(P') \leq w_{v'}(S') \Rightarrow \sum_{P \in \pi(v, S)} w'_v(P) \leq w'_{v'}(S)$, so the Tree condition holds. Finally, take any path $Q \in \pi(v)$. Case 1: The payoff to $v$ in the personalized equilibrium is at least $q_v(Q) + 1$. In this case, we know that $v$ puts a total of weight 1 on edges with payoff at least $q_v(Q) +1$, or $\sum_{P': u_v(P') \geq q_v(Q) + 1} w_v(P') = 1 \Rightarrow \sum_{P: P \geqprefer_v Q} w_v(P') = 1 \Rightarrow \sum_{P: P \geqprefer_v Q} w'_v(P) = 1$, so condition (S1) holds. Case 2: The payoff to $v$ in the personalized equilibrium is less than $q_v(Q) + 1$. Since this is a personalized equilibrium, it cannot be possible for $v$ to move some weight off a lower paying hyperedge onto a higher paying hyperedge. This includes moving weight from any of the edges in the equilibrium with payoff less than $q_v(Q) + 1$ to the edge $Q'$. By nature of the edges we've defined, if $P' \cap Q'$ for $P',Q' \in \pi(v)$, then either $P' \subset Q'$ or $Q' \subset P'$. This means
that there is some $S \in Q' (S \in \pi(v')$ such that $\sum_{R': S \in R'} w_v(R') = w_{v'}(S')$ and for all $R': S \in R'$, if $w_v(R') > 0$ then $q_v(R) \geq q_v(Q)$. So, $\sum_{R \in \pi(v, S)} w_v(R') = w_{v'}(S') \Rightarrow \sum_{R \in \pi(v, S)} w'_v(R) = w'_{v'}(S)$, and for all $R \in \pi(v, S)$ with $w'_v(R) > 0$, $R \geqprefer_v Q$, as required for condition (S2).

Next, assume $w'$ is a fractionally stable solution. We can assign weights $w_v(P') = w'_v(P)$, $w_v(N) = 1 - \sum_{P \in \pi(v)} w_v(P)$. The Unity condition ensures that $\sum_{P \in \pi(v)} w'_v(P) \leq 1$, $w_v(N) \geq 0$ and we have a set of weights that sum to 1 for any player $v$. The Tree condition says that $\sum_{P \in \pi(v, S)} w'_v(P) \leq w'_{v'}(S)$ for any $S \in \pi(v')$, which gives $\sum_{P': S \in P'} w_v(P') \leq w_{v'}(S')$, as required for a feasible solution. Finally, we must verify that $w_v$ is a best response for player $v$. Let $w^*$ be the best response weight function for $v$, and for the sake of contradiction, assume $w^*$ gives a better total payoff. Look at the edge $P'$ with the highest $q_v(P)$ such that $w^*_v(P') > w_v(P')$. By nature of the edges we've defined, if $P' \cap Q'$ for $P',Q' \in \pi(v)$, then either $P' \subset Q'$ or $Q' \subset P'$. Therefore, for all edges $P''$ with $q_v(P'') > q_v(P')$, if $w^*_v(P'') < w_v(P'')$, then we could increase $w^*_v(P'')$ and improve the payoff, so $P'$ is the highest utility edge in which $w_v$ and $w^*_v$ differ. Now look at edge $P'$ with weights $w$ in the fractional stable paths problem. Since $w^*_v(P') > w_v(P')$ and $w^*_v(P'') = w_v(P'')$ for all $P''$ with higher payoff than $P'$, then for all $S \in P'$ ($s \in \pi(v')$ for some $v'$),$\sum_{R': S \in R', q_v(R) > q_v(P)} w_v(R') < w_{v'}(S') \Rightarrow \sum_{R \in \pi(v, S), q_v(R) > q_v(P)} w'_v(R) < w'_{v'}(S)$, so condition (S2) is not satisfied. However, since $v$ puts less weight on edges with payoff at least as high as the payoff for $P'$, the total payoff to $v$ is $< q_v(P) + 1$. Therefore, $\sum_{R': q_v(R) \geq q_v(P)} w_v(R') < 1$, so $\sum_{R \geqprefer_v P} w'_v(R) < 1$, so condition (S1) is also not satisfied. This means that $w'$ was not a fractionally stable solution, contradicting our assumption. So $w$ must have been a best response weighting for each $v$.


==> pe_characterization.tex <==
\BfPara{A solution to the program is an exact personalized
  equilibrium} Assume we have a solution to
Equation~\ref{lp_with_mins} that is not a personalized
equilibrium. The first two constraints ensure that our solution is a
feasible weight assignment for the game. Therefore, there must be some
player $i$ who is not playing a best response. Take some better
response, in which player $i$ plays weights $w_i^*(e)$, and let
$\delta(e) = w^*_i(e) - w_i(e)$.

Let $F$ be the subset of $E_i$ such that $\delta(e) < 0$ (that is,
player $i$ puts more weight on each edge in $F$ in the original
response than in the best response). Since $w_i^*$ has a strictly
higher total utility for player $i$ than $w_i$, we know that $\sum_{e
  \in E_i} w^*_i(e) u_i(e) > \sum_{e \in E_i} w_i(e) u_i(e)$, which
implies that $\sum_{e \in E_i} \delta(e) u_i(e) > 0$.  Since both $w_i$
and $w^*_i$ were feasible weights, it must be true for any strategy
$s$ that $\sum_{e:s \in e} w_i(e) = \sum_{e: s \in e} w^*_i(e)
\Rightarrow \sum_{e: s \in e} \delta(e) = 0$.

By our definition of $F$, $\delta(e) < 0$ for all $e \in F$ and
$\delta(e) \geq 0$ for all $e \notin F$. Therefore, $F$ and $i$ obey
all the constraints of linear program \ref{non_optimal_lp}, so since
$w_i(e)$ obeyed program \ref{lp_with_mins}, we know that $\min_{e \in
  F} w_i(e) = 0$. Thus, there exists some edge $f \in F$ such that
$w_i(f) = 0$. But then $0 > \delta(f) = w^*_i(f) - w_i(f) = w^*_i(f)$,
contradicting the fact that $w^*_i$ was a feasible best response for
player $i$.  
\smallskip

\BfPara{Any personalized equilibrium is a solution to the program}
Assume we have a personalized equilibrium that does not satisfy some
constraint of the program. Let $w_i(e)$ be the weight placed by player
$i$ on edge $e$ in this equilibrium. The first three constraints
are the definition of a feasible weight assignment. Therefore, assume
this equilibrium does not satisfy the $\min$ constraint for some
player $i$ and some subset $F \subseteq E_i$ for which LP
\ref{non_optimal_lp} is feasible.

Consider a solution $\delta$ for LP \ref{non_optimal_lp} for this $i$
and $F$. Let $M = \frac{\min_{e \in F} |w_i(e)|}{\max_{e \in F}
  |\delta(e)|}$, and let $\delta'(e) = \delta(e) \cdot M$. $M$ is a
well-defined positive number since (1) the $\min$ constraint was not
satisfied, and (2) LP \ref{non_optimal_lp} specifies that $\delta(e) <
0$ for all $e \in F$. We know that $F$ is non-empty because the first constraint implies there is some $\delta > 0$, and combining this with the second constraint implies there is also some $\delta < 0$. Furthermore, for all $e$ with $\delta(e)<0$
(i.e., for all $e \in F$), $|\delta'(e)| \leq w_i(e)$. Now, consider
the alternate assignment for player $i$ specified by $w^*_i(e) =
w_i(e) + \delta'(e)$.  By the second constraint of LP
\ref{non_optimal_lp} and the fact that $|\delta'(e)| \leq w_i(e)$ for
all $e$ with $\delta(e) <0$, this is still a valid weight
assignment. By the first constraint of LP \ref{non_optimal_lp}, this
gives a strictly higher total utility for player $i$. Therefore,
weights $w_i(e)$ did not give a best response for player $i$, so we
did not have a personalized equilibrium, contradicting our assumption
and completing the proof.


==> pe_rational.tex <==
In Theorem \ref{thm:personalized_lp}, we showed that any personalized
equilibrium is a solution to a linear program plus additional $\min$
constraints, in which all coefficients are rational.  By Theorem
\ref{thm:exist}, this program has at least one solution. Now, we can
rewrite this as a union of many linear programs as follows. Let $F_1,
\ldots, F_{\alpha}$ be the set of all improvement sets. We can write
$\prod_{i=1}^{\alpha} |F_i|$ linear programs, each consisting of the first
three constraints from program \ref{lp_with_mins} as well as the
$\alpha$ constraints [$e_1 = 0$ for some $e_1 \in F_1$], [$e_2 = 0$
  for some $e_2 \in F_2$], $\ldots$, [$e_{\alpha} = 0$ for some
  $e_{\alpha}$ in $F_{\alpha}$]. We can create one LP for each
such combination of one edge from each improvement set, or
$\prod_{i=1}^{\alpha} |F_i|$ LPs. Since the union of these linear programs
is exactly the same as the program in Theorem
\ref{thm:personalized_lp}, and since (by Theorem \ref{thm:exist}) the
program in Theorem \ref{thm:personalized_lp} has at least one
solution, we know that at least one of these linear programs has a
solution. Any feasible LP with rational coefficients will have a
rational solution. Therefore, there will be a personalized equilibrium
with all rational weights.


==> pref_to_fspp.tex <==
We are given a preference game over player set $[n]$, including preference relation $\geqprefer_i$ for all $i \in 1 \ldots n$. We will convert this into a fractional stable paths problem. Create a node $v_i$ for each $i$. Also create a universal destination node $d$. For all $i$, define $P_{ii} = $ the path $(v_i, d)$. For all $i, j$, define $P_{ij} = $ the path $(v_i, v_j, d)$. Let $\pi(v_i)$ (the set of preferred paths for $v_i$) = $\{P_{ij}: j \geqprefer_i i\}$. If $k \geqprefer_i j$, then $P_{ik} \geqprefer_i P_{ij}$.

Let $w_i(j)$ refer to the amount of weight placed by node $v_i$ on path $P_{ij}$ in a fractional SPP solution, and let $w_i(i)$ be the amount of weight placed by $i$ on path $P_{ii}$. Now we will show that $w$ is a fractional stable paths solution if and only if $w$ defines an equilibrium of the preference game.

\BfPara{$w$ is a fractional stable paths solution $\Rightarrow$ $w$ is an equilibrium of the preference game.}
By the unity condition, for each $i$, $\sum_{j: P_{ij} \in \pi(v_i)} w_i(j) \leq 1 \Rightarrow \sum_j w_i(j) \leq 1$. $P_{ii}$ starts at $v_i$, and there is no proper final suffix of $P_{ii}$, so condition (S1) must apply for $P_{ii}$. Therefore, $\sum_{j: P_{ij} \in \pi(v_i)} w_i(j) = \sum_j w_i(j) = 1$, as required for the preference game. By the tree condition, for any $i, j$, $\sum_{P \in \pi(v, P_{jj}}$ weight on $P \leq w_j(j) \Rightarrow w_i(j) \leq w_j(j)$. So $w$ is a feasible weight assignment for the preference game.

Now suppose for contradiction that $w$ is not lexicographically maximal (with respect to $w_{-i}$) for player $i$ in the preference game. Then, there is some feasible weight assignment $w'$ and some $j$ such that $\sum_{k \geqprefer_i j} w_i(k) < \sum_{k \geqprefer_i j} w'_i(k)$.  Take the lexicographically maximal such $w'$ and the highest preference such $j$ (from $i$'s preference list).  By this choice of $w'$ and $j$, $\sum_{k \gtprefer_i j} w_i(k) = \sum_{k \gtprefer_i j} w'_i(k)$, so $\sum_{k \eqprefer_i j} w_i(k) < \sum_{k \eqprefer_i j} w'_i(k)$. There must be some $j'$ with $j' \eqprefer_i  j$ such that $w_i(j') < w'_i(j')$.
Consider path $P_{ij'}$. (S2) is not true by our choice of $j'$ and the fact that $w'$ was a feasible solution (so $w'_i(j') \leq w_{j'}(j')$). However, since $\sum_{k \eqprefer_i j'} w_i(k) < \sum_{k \eqprefer_i j'} w'_i(k)$, there must be some path $P_{ik}$ such that $k \ltprefer_i j'$ with $w_i(k) > 0$. So (S1) is also not true, and $w$ was not a stable solution - a contradiction.

\medskip

\BfPara{$w$ is an equilibrium of the preference game $\Rightarrow$ $w$ is a fractional stable paths solution.}
We know that $\sum_j w_i(j) = 1$ for all $i$. This immediately satisfies the unity condition. Since $w$ is a feasible set of weights for the preference game, $w_i(j) \leq w_j(j)$ for all $i, j$. This means that the weight placed on $P_{ij}$ is at most the weight placed on $P_{jj}$. Since $P_{ij}$ is the only path from $v_i$ that passes through node $v_j$, the tree condition holds. Now consider any path $P_{ij}$ from node $i$. Case 1: $w_i(j) = w_j(j)$. In this case, condition (S2) is satisfied.  Case 2: $w_i(j) < w_j(j)$. Because $w$ was lexicographically maximal, any weight assignment $w'$ with $\sum_{k \geqprefer_i j} w'_i(k) \geq \sum_{k \geqprefer_i j} w_i(k)$ must be infeasible. We said that $w_i(j) < w_j(j)$, so it is only possible for all such $w'$ to be infeasible if $\sum_{k \geqprefer_i j} w_i(k) = 1$. Then $\sum_{k \ltprefer_i j} w_i(k) = 0$, so (S1) is satisfied.

